Making the Invisible Visible: Action Recognition Through Walls and Occlusions

Understanding people's actions and interactions typically depends on seeing them. Automating the process of action recognition from visual data has been the topic of much research in the computer vision community. But what if it is too dark, or if the person is occluded or behind a wall? In this paper, we introduce a neural network model that can detect human actions through walls and occlusions, and in poor lighting conditions. Our model takes radio frequency (RF) signals as input, generates 3D human skeletons as an intermediate representation, and recognizes actions and interactions of multiple people over time. By translating the input to an intermediate skeleton-based representation, our model can learn from both vision-based and RF-based datasets, and allow the two tasks to help each other. We show that our model achieves comparable accuracy to vision-based action recognition systems in visible scenarios, yet continues to work accurately when people are not visible, hence addressing scenarios that are beyond the limit of today's vision-based action recognition.

==> source/experiment.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth, height=0.6\linewidth]{main-result}
\end{center}
\caption{\footnotesize{Qualitative Results. The figure shows \name's output in various scenarios.}}\label{fig:main}
\end{figure*}


\section{Experiments}

\input{source/dataset}

\subsection{Setup}
\vskip 0.06in\noindent
\textbf{Metric.}
As common in the literature on video-based action detection  \cite{lin2017single,zhao2017temporal,Heilbron_2015_CVPR} and skeleton-based temporal action detection  \cite{liu2017pku,li2017skeleton,li2018co}, we evaluate the performance of our model using the mean average precision (mAP) at different intersection-over-union (IoU) thresholds $\theta$. We report our results on mAP at 0.1 and 0.5 IoU thresholds.

%\vskip 0.06in\noindent
%\textbf{Baselines.} For scenarios without occlusions, we compare RF-action with HCN \cite{li2018co}, which uses is the current state-of-the-art model for skeleton-based action recognition. \red{We use the 3D skeleton sequences from  our multi-view camera system as inputs of the baseline models.} We also add our spatial-temporal attention module and multi-proposal module to their architecture for a fair comparison. To compare with approaches from wireless communities, we follow the Aryokee \cite{tian2018rf} pipeline and detect actions directly from RF signals without skeleton as intermediate representation.

\vskip 0.06in\noindent
\textbf{Ground Truth Labels.}
To perform end-to-end training of our proposed \name\ model, we need two type of ground truth labels: 3D human skeletons to supervise our intermediate representation, and action start-end time and category to supervise the output of our model. The 3D skeletons are triangulated using AlphaPose and the multi-view camera system descried earlier. As for actions' duration and category, we manually segment and label the action of each person using the multi-view camera system.

\subsection{Qualitative Results}
\autoref{fig:main} shows qualitative results that illustrate the output of \name\ under a variety of scenarios.  The figure shows that detects actions and interactions, works correctly when different people perform different actions simultaneously, and an deal with occlusions and poor lighting. Hence, it addresses multiple challenges for today's action recognition systems. 


\subsection{Comparison of Different Models}

We compare the performance of \name\ to the state-of-the-art models for skeleton-based action recognition and RF-based action recognition. We use HCN as a representative of a top performant skeleton-based action recognition system in computer vision. It currently achieves the best accuracy on this task.  We use Aryokee~\cite{tian2018rf} as a representative of the state-of-the-art in RF-based action recognition. To our knowledge, this is the only past RF-based action recognition system that performs action detection in addition to classification.\footnote{The original Aryokee code is for two classes. So we extended to support more classes.} All models are trained and tested on our RF action recognition dataset. Since HCN takes skeletons as input (as opposed to RF signals) we provide it with the intermediate skeletons generated by \name. This allows us to compare \name\ to HCN in terms of action recognition based on the same skeletons. 

\begin{table}[htbp]
  \small
	\centering
	\begin{tabular}{ccccc}
		\hline
		\multirow{3}{*}{Methods} & \multicolumn{2}{c}{Visible scenes} & \multicolumn{2}{c}{Through-wall}\\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
		& \multicolumn{2}{c}{mAP} & \multicolumn{2}{c}{mAP}\\ 
		& $\theta$=0.1 & $\theta$=0.5 & $\theta$=0.1 & $\theta$=0.5 \\
		\hline
		\name\ & \textbf{90.1} & \textbf{87.8} & \textbf{86.5} & \textbf{83.0}\\
		HCN \cite{li2018co} & 82.5 & 80.1 & 78.5 & 75.9  \\
		Aryokee \cite{tian2018rf} & 78.3 & 75.3 & 72.9 & 70.2 \\
		\hline
	\end{tabular}
  \vspace{-5pt}
	\caption{\footnotesize{Model Comparison on RF-MMD dataset. The table shows mAP in visible and through-wall scenarios under different IoU threshold $\theta$. Since HCN operates on skeletons, and for fair comparison, we provide it with the RF-based skeletons generated by \name.}	}
  \label{tab:ap_main}
\end{table}


 \autoref{tab:ap_main} shows the results for testing on visible scenes and through-wall scenarios, with wireless signals as the input.  As shown in the table, \name\ outperforms HCN in both testing conditions. This shows the effectiveness of our proposed attention and multi-proposal modules. From the result we can also see that \name\ outperforms Aryokee by a large margin on both visible and through-wall scenarios. This shows that the additional supervision from the skeletons, as well as \name\ neural network design are important for delivery accurate performance using RF data. 



\subsection{Comparison of Different Modalities}
Next we investigate the performance of \name\ when operating on RF-based skeletons versus vision-based skeletons. 
We train \name\ on the training set, as before. However, when performing inference, we either provide it with the input RF signal from the test set, or we provide it with the visible ground truth skeletons obtained using our camera system. 
\autoref{tab:ap_main_vision} shows the results for different input modalities. The table shows that for visible scenes, operating on the ground truth skeletons from the camera system leads to only few percent improvement in accuracy. This is an interesting result since the RF-skeletons are trained with the vision-based skeleton as ground truth. Further, 
as we described in our experimental setting, the camera-based system uses 10 view points to estimate 3D skeletons 
while only one wireless device is used for action recognition based on RF. This results demonstrates that RF-based action recognition can achieve a performance close to a carefully calibrated camera system with 10 view points. The system continues to work well in through-wall scenarios though the accuracy is few percent lower due to the signal experiencing some attenuation as it traverse walls. 

\begin{table}[htbp]
  \small
	\centering
	\begin{tabular}{ccccc}
		\hline
		\multirow{3}{*}{Method / Skeletons } & \multicolumn{2}{c}{Visible scenes} & \multicolumn{2}{c}{Through-wall}\\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
		& \multicolumn{2}{c}{mAP} & \multicolumn{2}{c}{mAP}\\ 
		& $\theta$=0.1 & $\theta$=0.5 &  $\theta$=0.1 & $\theta$=0.5 \\
		\hline
		\name\ / RF-MMD & 90.1 & 87.8 & 86.5 & 83.0\\
		\name\ / G.T. Skeleton & 93.2 & 90.5 & - & - \\
		\hline
	\end{tabular}
  \vspace{-5pt}
	\caption{\footnotesize{\name's Performance (mAP) with RF-Based Skeletons (RF-MMD) and Vision-Based Skeleton (G.T. Skeleton) under different IoU threshold $\theta$.}}
  \label{tab:ap_main_vision}
\end{table}


\subsection{Action Detection}

In \autoref{fig:detection-result}, we show  representative example of our action detection results on the test set. Two people are enrolled in this experiment. They sometimes do actions on their own, and sometimes interact with each other. The first row shows the action duration for the first person, the second row shows the action duration of the second person, and the third row shows the interactions between them. Our model can detect both the actions of each person and the interactions between them with high accuracy. This result clearly demonstrates that our multi-proposal module has good performance in scenarios where multiple people are independently performing some actions  or interacting with each other. 

\begin{figure}[htbp]
\centering
\includegraphics[width=\linewidth]{detection-result}
\caption{\footnotesize{Example of action detection results on the test set, where two people are doing actions as well as interacting with each other. Ground truth action segments are drawn in blue, while detected segments using our model are drawn in red. The horizontal axis refers to the frame number.}}	\label{fig:detection-result}
\end{figure}



We also show the results for action detection with different number of subjects in the scene (\autoref{fig:people}). We can see  that the detection accuracy drops when the number of people increases. This performance drop is due to the low resolution of RF signal. Since the signals reflected from different people can interfere with each other, the accuracy of wireless systems typically decrease as the number of people increases. However, the intermediate skeleton representation minimizes this interference and our system still shows good performance even when there are 3 people in the scene. 

\begin{figure}[htbp]
\centering
\subfigure{\includegraphics[width=0.47\linewidth]{people-result-10}}
\subfigure{\includegraphics[width=0.47\linewidth]{people-result-50}}

\caption{\footnotesize{mAP at IOU threshold $\theta=0.1$ and $\theta=0.5$ with different number of people.}}\label{fig:people}
\end{figure}


\subsection{Ablation Study}
We also conduct extensive ablation studies to verify the effectiveness of each key component of our proposed approach. For simplicity, the following experiments are conducted on the visible scenes in RF-MMD and mAP are calculated under 0.5 IoU threshold.
\vskip  0.06in \noindent
\textbf{Attention Module. }
We evaluate the effectiveness of our proposed spatial-temporal attention module in \autoref{tab:ap_attention}. We show action detection performance with or without our attention module on both RF-MMD and PKU-MMD. The results show that our attention is useful for both datasets, but is especially useful when operating on RF-MMD. This is because skeletons predicted from RF signals can have some errors and inaccurate joints. We also conduct experiments on the NTU-RGB+D ~\cite{shahroudy2016ntu} dataset. Unlike PKU-MMD and RF-MMD which allow for action detection, this dataset is valid only for action classification. 
The table shows that our attention module is useful in this case too. 

\begin{table}[htbp]
  \small
	\centering
 	\begin{tabular}{ccc}
 		\hline
		Datasets (Metric)& \name\ & \name\ w/o Attention \\
 		\hline
 		RF-MMD (mAP) & \textbf{87.8} & 80.1 \\
		PKU-MMD (mAP) & \textbf{92.9}/\textbf{94.4} & 92.6/94.2 \\
		NTU-RGB+D (Acc) & \textbf{86.8}/\textbf{91.6} & 86.5/91.1 \\
 		\hline
 	\end{tabular}
  \vspace{-5pt}
	\caption{\footnotesize{Performance of \name\ on Different Datasets With and Without Attention. For PKU-MMD and NTU-RGB+D (cross subject / cross view), we only test the action recognition neural network (without the skeleton generation network).}}
  \label{tab:ap_attention}
\end{table}

\textbf{Multi-Proposal Module.}
We propose a multi-proposal module to enable multiple action prediction at the same time. We evaluate our model's performance with or without the multi-proposal module. As shown in \autoref{tab:ap_multi_proposal}, the added multi-proposal module significantly increase the performance. This is because our dataset includes a lot of instances when people are performing different actions at the same time. Our model will get very poor accuracy at these scenarios with single-proposal, while with multi-proposal our model can achieve a much higher performance.

\begin{table}[htbp]
  \small
	\centering
	\begin{tabular}{cc}
		\hline
		Methods & RF-MMD \\
		\hline
		Multi-Proposal & 87.8 \\
		Single-Proposal & 65.5 \\
		\hline
	\end{tabular}
  \vspace{-5pt}
	\caption{\footnotesize{Benefits of Multi-proposal Module. The table shows that adding multi-proposal module significantly improves the performance on RF-MMD}}
  \label{tab:ap_multi_proposal}
\end{table}


\textbf{Multimodal Training.}
As explained earlier, the use of skeletons as an intermediate representation allows the model to learn from both RF datasets and existing vision-based skeleton datasets. To  illustrate this advantage, we perform multimodal training by adding PKU-MMD's training set into the training of our RF-Action model. More specifically, we use our dataset to train the whole \name\ end-to-end model, and use the PKU-MMD dataset to train \name's activity detection model. These two datasets are used alternatively during training. As shown in \autoref{tab:ap_joint}, comparing the detection results with the model trained on either dataset separately, we find multimodal training can increase the model performance since it introduces more data for training and therefore can get better generalization ability. 

\begin{table}[htbp]
  \small
	\centering
	\begin{tabular}{ccc}
		\hline
		Training set / Test set & RF-MMD & PKU-MMD \\
		\hline
		RF-MMD+PKU-MMD & \textbf{87.8} & \textbf{93.3}/\textbf{94.9} \\
		RF-MMD & 83.3 & 60.1/60.4 \\
		PKU-MMD & 77.5 & 92.9/94.4 \\
		\hline
	\end{tabular}
  \vspace{-5pt}
	\caption{\footnotesize{Benefits of Multimodal Training. The table shows that adding PKU-MMD to the training set significantly improves the performance on RF-MMD. The mAP of RF-MMD+PKU-MMD on RF-MMD are achieved using the cross subject training set of PKU-MMD. Using only RF-MMD for training has pool performance on PKU-MMD because the action set of RF-MMD is a subset of PKU-MMD's action set.}}
  \label{tab:ap_joint}
\end{table}


\textbf{End-to-End Model.}
\name\ uses an end-to-end model where the loss of action recognition is propagated through the skeleton generation network. Here we show that such an end-to-end approach improves the skeleton itself.  \autoref{tab:ap_e2e} reports the average error in skeleton joint location, for two systems: our end-to-end model and an alternative model where the skeleton is learned separately from the action --i.e., the action loss is not propagated through the skeleton generation network. The table shows that the end-to-end model not only improves the performance of the action detection task, but also reduces the errors in estimating the location of joints in RF-based skeletons. This is because the action detection loss provides regularization for 3D skeletons generated from RF signals. 

\begin{table}[htbp]
  \small
	\centering
	\begin{tabular}{ccc}
		\hline
		Methods & mAP & Skeleton Err. (cm) \\
		\hline
		end-to-end & 87.8 & 3.4 \\
		separate & 84.3 & 3.8 \\
		\hline
	\end{tabular}
  \vspace{-5pt}
	\caption{\footnotesize{mAP and intermediate 3D skeleton error on testing data with and without end-to-end training.}}
  \label{tab:ap_e2e}
\end{table}


%\section{Limitations}
%\name\ uses RF signals to recognize human actions through walls and occlusions. However, RF signals and the solution that we present herein have some limitations. Since the human body is opaque at the frequencies of our RF signals, our signals can be occluded by other people, i.e., inter-person occlusion, or the person doing actions himself, i.e., self-occlusion. As a result, our system is limited when there are too many people at the same time, or the person doing actions occludes his important joints by his body, e.g. when someone is playing phones back to our device. We conduct a more thorough analysis of our failure cases in Appendix XXX.


==> source/intro.tex <==
\section{Introduction}
Human action recognition has attracted much interests from the research community. It has broad applications in video surveillance, game control, human behavior analysis etc. Action recognition is defined as detecting and classifying human actions from some time series (video frames, human skeleton sequences, etc). Over the past few years, the progress of deep learning, especially CNNs, helped improve video action recognition at an amazing speed. Nonetheless, most camera-based approaches suffer from severe performance drop when the subjects are occluded. Previous works tackled this problem by changing camera view point or interpolating frames over time. However, such approaches fail when the camera is fixed or the person is fully occluded for a relatively long period, e.g., the person walks into another room.

In this paper, we develop a novel approach to detect and recognize human actions from wireless signals. Radio signals in the WiFi range  traverse walls and occlusions and reflect off human bodies. Our approach leverages such radio signals to recognize human actions through occlusions and under poor light conditions. Recent works in wireless systems tend to leverage this property to detect human movement or poses behind walls \cite{zhao2018rf, zhao2018through}. However, previous approaches can only work under limited conditions: human are usually walking or standing, which means the skeletons are quite regular. Subtle movements like lifting arms may not be captured appropriately which makes it inadequate to capture detailed human actions. There are also works to recognize human actions directly from wireless signals. However, their algorithms are often with limited action set ($<$10 classes), poor generalization to new environments, and incompatibility with multi-person scenario. These approaches are not comparable to the performance achieved by vision-based models. As a result, leveraging wireless signals to recognize accurate and detailed human actions remains an open-problem.

\begin{figure}[t]
	\centering
	\subfigure[hand shaking]{
		\includegraphics[width=0.47\linewidth]{teaser-shaking}\label{fig:image-vis}
	}
	\subfigure[throw]{
		\includegraphics[width=0.47\linewidth]{teaser-throw}\label{fig:skeleton-vis}
	}
\caption{\footnotesize{The figure shows two test cases of our system. The left one shows two people are handshaking, while one of them are behind the wall. The right one shows one person in the dark are throwing a knife to another person. In both cases our wireless system is able to detect the actions while traditional camera-based vision system cannot.\red{to replace}}}	\label{fig:teaser}
\end{figure}


To tackle this problem, we present RF-Action, a multimodal end-to-end deep neural network based approach to recognize human actions directly from wireless signals, which is robust under occlusion or dark conditions. \autoref{fig:teaser} shows two examples of RF-Action under these conditions. The left one shows two people handshaking, while one of the people are behind the wall. In this case, we cannot tell what the right person are doing simply from visual input, while wireless signal can reveal that they are actually shaking hands. The right one shows one person in the dark are trying to throw a knife to another person. Again while camera cannot capture the person hand in the dark, the wireless signals can capture him and alarm possible malicious action.

Our model uses 3D human skeletons as a latent representation to provide additional supervision on the skeletons. Using human skeletons as an intermediate representation has several advantages: (1) It provides our model with the ability to train with both RF dataset and vision dataset, as long as we can extract skeletons from the dataset. (2) Human skeletons are quite robust to background noises, so it can be viewed as a regularization and improve the generalization ability of our model between different environments. Performing end-to-end training from wireless signals to activities helps improve performance on both action recognition and pose estimation. It helps to generate more accurate and continuous skeletons which can help with accurate action recognition.


To train and evaluate our method, we collect an action detection dataset from different environments with a wireless device and a camera system. The dataset contains 30 subjects performing random actions chosen from a list of 40 different daily actions. We record wireless signals from the radio device and images from the camera system simultaneously, and manually label the start end time of each action. Furthermore, the camera system generates the ground truth 3D skeleton for the supervision on the intermediate skeleton representation of our model.

Our model handles a more general scenario of multi-person action recognition, and also takes into account the possible misprediction of RF-generated human skeletons. Unlike standard datasets such as PKU-MMD and NTU RGB+D \cite{liu2017pku, shahroudy2016ntu}, in our dataset different people may perform different actions simultaneously. Previous models do not deal with this properly since they can only predict one action at a time. Furthermore, the skeletons generated from RF signals can mispredict  body joints. This noise will severely degrade the performance of action detection models trained on those clean standard visual dataset.

To tackle these problems, we propose a multi-proposal module to handle the multi-person action recognition scenario, and a spatial-temporal attention module to improve the action recognition performance from skeletons generated by wireless signals. Our results show that these two modifications not only improve RF-based action recognition by a large margin, but also can be easily adopted by previous skeleton-based action recognition algorithms to achieve better performance on standard vision-based dataset. 

Our experiments show that under conditions with no occlusions, our RF-action can achieve \textcolor{red}{87.8} average precision (AP) on our test set. Under partially occluded or through-wall conditions, RF-Action can still achieve an AP of \textcolor{red}{83.0}. 

Our result also shows that performing multimodal training can improve the action detection performance on both visual and wireless modalities. Training our model with both our dataset and PKU-MMD dataset, we observe a performance increase on AP from \textcolor{red}{86.3} to \textcolor{red}{87.8} for wireless validation set, and from \textcolor{red}{92.6} to \textcolor{red}{92.6} for vision validation set.



==> source/method-1.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{model}
\end{center}
\caption{Our model architecture. Our model first extract 3D skeleton estimations for each person from raw wireless signal inputs. It then perform action recognition on the extracted skeletons.}\label{fig:method}
\end{figure*}


\section{Methods}
\name\ is  an end-to-end neural network model that can detect human actions through occlusion and in bad lighting. The model architecture is illustrated in \autoref{fig:method}. As shown in the figure, the model takes wireless signals as input, generates 3D human skeletons as an intermediate representation, and recognizes actions and interactions of multiple people over time. 

The figure further shows that \name\ can also take 3D skeletons generated from visual data. This allows \name\ to train with existing 3D skeleton datasets. The model can also perform inference on either data modality or both. 
For example, consider the handshake in \autoref{fig:teaser} where one person is visible and the other is hidden. If the model is given only RF signals, it  will generate two sequences of 3D skeletons and recognize the action purely based on RF data.  If the model is given both the RF signals and the 3D skeleton sequence of the visible person extracted from RGB-D or a camera system, the model can use RF to generate the skeleton sequence for the hidden person and combine it with the vision-based skeleton sequence of the visible person to produce an action label.\footnote{The model can use the confidence level to decide whether to accept the RF-based or vision-based skeleton sequence for the visible person.}
 
In the rest of this section, we will describe how we transform wireless signals to 3D skeleton sequences, and how we infer actions from such skeleton sequences --i.e., the yellow and green boxes in \autoref{fig:method}. Transforming visual data from a camera system or RBG-D camera to 3D skeletons follows the standard approaches in the literature~\cite{XXX,XXX,XXX,XXX}. 


\subsection{Radio Signal to Skeleton}
We adopt the top-down detection architecture from \cite{zhao2018rf} to generate multi-person 3D skeletons from RF signals. Specifically, we have a neural network model that uses spatio-temporal convolutions. It takes as inout a 3-second window of RF signals (90 frames of horizontal and vertical heatmaps). Similar to Faster R-CNN \cite{ren2015faster}, our input first goes through a feature network to extract features from the input RF signals. Since the  convolution operation does not change the spatial distribution of the input, we will obtain two kinds of feature maps, one from the horizontal RF heatmaps and another from vertical RF heatmaps. A region proposal network (RPN) is applied on the horizontal feature maps to obtain several proposals for possible skeleton bounding  boxes. After that, the extracted proposals are fed into a 3D pose estimation subnetwork to extract 3D skeletons from each of them. 

\subsection{Skeleton to Action}
After we generate 3D skeletons from  raw wireless signals, we can start to perform action detection on these skeletons. We first associate the skeletons across time to get multiple skeleton sequences, each from one person. Then we apply our skeleton-based action recognition algorithms on these skeleton sequences. Specifically, we leverage the two-stream hierarchical co-occurrence network (HCN) architecture to extract spatio-temporal features, as well as joint co-occurrences~\cite{zhu2016co} .  We process each skeleton sequence with HCN to extract high-level features.  We pass these feature to a temporal proposal network to extract time windows that correspond to an action.   Our temporal proposal network follows the design in \cite{zhu2016co} which adapt the Faster R-CNN \cite{girshick2015fast} framework to the temporal dimension. 
After cropping and resizing the corresponding latent feature, we input it into a classification network. The classification network is responsible for two things: First, it refines the temporal proposal result and do a 2-way classification to determine whether this duration contains an action or not. Second, it predicts the action class of the corresponding temporal duration.

\textbf{Multi-proposal Module} 
Previous approaches for skeleton action recognition cannot handle the scenario where multiple people performing different action simultaneously, since their model can only predict one action label for each duration. If one person is sitting while other other two people are shaking hands, previous model can not predict both actions. We tackle this problem with a multi-proposal module. Specifically, denote $N$ to be the maximum possible number of persons appearing at the same time. To consider the actions of everyone, we first stack all body joints from every person to be the input for our model, for scenario with $<N$ person performing actions, we simply pad zero. After extracting latent features from each one of the skeleton sequences, instead of performing max-pooling over $N$ features, our temporal proposal subnetwork propose $N+C_N^2$, corresponding to $N$ single-person actions and $C_N^2$ possible interactions between different person. After proposal, we adopt a rank pooling strategy between interact and single person actions. For instance, if there are both predictions for 'pointing to something'(single person) and 'pointing to someone'(interaction) at the same time, our final prediction would be 'pointing to someone'.
Our multi-proposal module can be easily adapt to most of the previous action detection frameworks to enable the model to predict multiple actions and interactions at the same time.


\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{attention}
\caption{Spatial-temporal attention module to pay different attention on different joints and time segments. \red{to replace}}	\label{fig:rf-heatmaps}
\end{figure}
\textbf{Spatial-Temporal Attention Module}
Skeletons predicted from wireless signals may not be as accurate as labeled by human. Also, different body joints may have different predict accuracies. To make our action detection model focus more on the body joint with higher prediction confidence, we propose a spatial-temporal attention module(STAM). Specifically, we define a learnable mask weight $W_m$, and convolve with latent features from spatial path $f_{si}$ and temporal path $f_{ti}$ and get the mask to apply on the feature.
$$Mask=Conv(concat(f_{si}, f_{ti}))$$
In this way, the mask could learn to provide different weights to different joints to get better action recognition performance.
In practice, we find the proposed attention module also helps the model to learn more representation features, since the learnt mask leverage information provided by both spatial path and temporal path, while the previous model only have have the two paths interact with each other with late fusion. Therefore, it helps to combine spatial and temporal representations more effectively, and would lead to better latent representations for the skeleton sequences. It could help to classify the actions which can be better disentangled by a mixture of spatial and temporal information, e.g. brushing hair and answering phone.
Our spatial-temporal attention module and also be easily adapted to most of the previous two-stream based neural network architectures for action recognition and other spatial-temporal modeling tasks, and our experiments show that it also helps increase the performance on benchmark action recognition datasets. 


\subsection{Multimodal End-to-end Training}
Our end-to-end architecture has 3D human skeleton as an intermediate representation, which makes us able to leverage previous skeleton based action recognition dataset easily. We train our model with different modalities in the following manner: For wireless signal datasets, gradients propagate through the whole model, and they are used to tune the parameters in both skeleton prediction module and action recognition module; For previous skeleton-based action recognition datasets, the gradients back propagate till the skeleton, and they are used to tune the parameters for the action recognition module. Indeed, datasets for action recognition from other modalities can also be leveraged, as long as we can extract skeletons from the inputs.


==> source/method-2.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{model}
\end{center}
\caption{\footnotesize{Our model architecture. Our model first extract 3D skeleton estimations for each person from raw wireless signal inputs. It then perform action recognition on the extracted skeletons.}}\label{fig:method}
\end{figure*}


\section{Method}
\name\ is  an end-to-end neural network model that can detect human actions through occlusion and in bad lighting. The model architecture is illustrated in \autoref{fig:method}. As shown in the figure, the model takes wireless signals as input, generates 3D human skeletons as an intermediate representation, and recognizes actions and interactions of multiple people over time. 
The figure further shows that \name\ can also take 3D skeletons generated from visual data. This allows \name\ to train with existing 3D skeleton datasets. 
%The model can also perform inference on either data modality or both. For example, consider the handshake in \autoref{fig:teaser} where one person is visible and the other is hidden. If the model is given only RF signals, it  will generate two sequences of 3D skeletons and recognize the action purely based on RF data.  If the model is given both the RF signals and the 3D skeleton sequence of the visible person extracted from RGB-D or a camera system, the model can use RF to generate the skeleton sequence for the hidden person and combine it with the vision-based skeleton sequence of the visible person to produce an action label.\footnote{The model can use the confidence level to decide whether to accept the RF-based or vision-based skeleton sequence for the visible person.}
 
In the rest of this section, we will describe how we transform wireless signals to 3D skeleton sequences, and how we infer actions from such skeleton sequences --i.e., the yellow and green boxes in \autoref{fig:method}. Transforming visual data from a camera system or RBG-D camera to 3D skeletons follows the standard approaches in the literature~\cite{XXX,XXX,XXX,XXX}. 


\subsection{Radio Signal to Skeleton}
We adopt the top-down detection architecture from \cite{zhao2018rf} to generate multi-person 3D skeletons from RF signals. Specifically, we have a neural network model that uses spatio-temporal convolutions. Each time, it takes as input a 3-second window of RF signals (90 frames of horizontal and vertical heatmaps). Similar to Faster R-CNN \cite{ren2015faster}, our input first goes through a feature network to extract features from the input RF signals. Since the  convolution operation does not change the spatial distribution of the input, we will obtain two kinds of feature maps, one from the horizontal RF heatmaps and another from vertical RF heatmaps. A region proposal network (RPN) is applied on the horizontal feature maps to obtain several proposals for possible skeleton bounding  boxes. After that, the extracted proposals are fed into a 3D pose estimation subnetwork to extract 3D skeletons from each of them. 

\subsection{Skeleton to Action}
After we generate 3D skeletons from raw wireless signals, we can start performing action detection on these skeletons. We first associate the skeletons across time to get multiple skeleton sequences, each from one person. Then we apply our skeleton-based action recognition algorithms on these skeleton sequences. We leverage a modified version of HCN \cite{zhu2016co} with additional attention module as our feature learning network, which is a two-stream hierarchical co-occurrence network architecture to extract spatio-temporal features, as well as joint co-occurrences \cite{zhu2016co}.

We then pass these feature extracted from our feature learning network to a multi proposal module to extract time windows that correspond to an action. Our multi proposal module consists of many proposal sub-networks. Each sub-network either takes in a feature from one person to detect actions proposals, or takes in two features from two people to detect interactions proposals. Each proposal sub-network follows the design in \cite{zhu2016co} which adapts the Faster R-CNN \cite{girshick2015fast} framework for temporal proposals extraction. 

Finally, after cropping and resizing the corresponding latent feature using the proposals from our multi-proposal module, we input each cropped action segment into a classification network. The classification network first refines the temporal proposal result by performing a 2-way classification to determine whether this duration contains an action or not. It then predicts the action class of the corresponding action segment.

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{attention}
\caption{\footnotesize{Spatial-temporal attention module to pay different attention on different joints and time segments.}}	\label{fig:rf-heatmaps}
\end{figure}

\subsubsection{Spatial-Temporal Attention Module}
Skeletons predicted from wireless signals may not be as accurate as labeled by human. Also, different body joints may have different predict accuracies. To make our action detection model focus more on the body joint with higher prediction confidence, we propose a spatial-temporal attention module(STAM). Specifically, we define a learnable mask weight $W_m$, and convolve with latent features from spatial path $f_{si}$ and temporal path $f_{ti}$ and get the mask to apply on the feature.
$$Mask=Conv(concat(f_{si}, f_{ti}))$$
In this way, the mask could learn to provide different weights to different joints to get better action recognition performance. We also add a multi-headed attention module \cite{vaswani2017attention} on the time dimension after the feature extraction to learn the attention on different timestamps.

Our proposed attention module helps the model to learn more representative features, since the learnt mask leverages information provided by both spatial path and temporal path, and the multi-headed attention helps the model to attend more on useful timestamps, while the previous model only have have the two paths interact with each other with late fusion. Our extensive experiments show that the spatial-temporal attention module not only helps increase the action detection accuracy on skeletons predicted from wireless signals, but also helps increase the performance on benchmark visual action recognition datasets. This further shows the proposed attention module helps to combine spatial and temporal representations more effectively, and would lead to better latent representations for the skeleton sequences.

\subsubsection{Multi-proposal Module} 
Most of previous action recognition datasets have only one action target at a time, regardless of the number of people presented. As a result, previous approaches for skeleton action recognition cannot handle the scenario where multiple people performing different action simultaneously. When there are multiple people in the scene, they typically simply do a max over features extracted from each of them, and forward the resulting combined feature to output one action. Therefore, they can only predict one action label at a time. If one person is sitting while other two people are shaking hands, previous model can not predict both of them.

However, in our dataset, when there are multiple people in the scene, they are free to do any actions or interact with each other at any time. So there are many scenarios where multiple people are doing actions and interacting simultaneously. We tackle this problem with a multi-proposal module. Specifically, denote $N$ to be the number of people appearing at the same time. Instead of performing max-pooling over $N$ features, our multi-proposal module output $N+{n\choose 2}$ proposals from these $N$ features, corresponding to $N$ possible single-person actions and ${n\choose 2}$ possible interactions between each two people. After proposal, we adopt a priority strategy between interact and single person actions. For instance, if there are both predictions for 'pointing to something' (single person) and 'pointing to someone' (interaction) at the same time, our final prediction would be 'pointing to someone'.

Our multi-proposal module enables us to output predicted action for each person at the same time. Also, adding the multi-proposal module will have no harm on previous datasets.

\subsubsection{Multimodal End-to-end Training}
Since we want to train our model in an end-to-end manner, we can no longer use $\arg\max$ to extract 3D keypoint locations. Therefore, we use a regressor to perform the function of the $\arg\max$ to extract the exact 3D locations of each keypoint. This makes the whole model becomes differentiable and therefore the action label can also act as a supervision on the skeleton prediction model.

Our end-to-end architecture uses 3D human skeleton as an intermediate representation which makes us able to leverage previous skeleton based action recognition dataset easily. We combine different modalities to train our model in the following manner: For wireless signal datasets, gradients propagate through the whole model, and they are used to tune the parameters of both the skeleton prediction model and the action recognition model; For previous skeleton-based action recognition datasets, the gradients back propagate till the skeleton, and they are used to tune the parameters for the action recognition module. As shown in the experiment session, these multi-modality training significantly increase the data diversity and improves the performance of our model.

==> source/method-3.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{model}
\end{center}
\caption{\footnotesize{Our model architecture. Our model first extract 3D skeleton estimations for each person from raw wireless signal inputs. It then perform action recognition on the extracted skeletons.}}\label{fig:method}
\end{figure*}


\section{Method}
\name\ is  an end-to-end neural network model that can detect human actions through occlusion and in bad lighting. The model architecture is illustrated in \autoref{fig:method}. As shown in the figure, the model takes wireless signals as input, generates 3D human skeletons as an intermediate representation, and recognizes actions and interactions of multiple people over time. 
The figure further shows that \name\ can also take 3D skeletons generated from visual data. This allows \name\ to train with existing 3D skeleton datasets. 
%The model can also perform inference on either data modality or both. For example, consider the handshake in \autoref{fig:teaser} where one person is visible and the other is hidden. If the model is given only RF signals, it  will generate two sequences of 3D skeletons and recognize the action purely based on RF data.  If the model is given both the RF signals and the 3D skeleton sequence of the visible person extracted from RGB-D or a camera system, the model can use RF to generate the skeleton sequence for the hidden person and combine it with the vision-based skeleton sequence of the visible person to produce an action label.\footnote{The model can use the confidence level to decide whether to accept the RF-based or vision-based skeleton sequence for the visible person.}
 
In the rest of this section, we will describe how we transform wireless signals to 3D skeleton sequences, and how we infer actions from such skeleton sequences --i.e., the yellow and green boxes in \autoref{fig:method}. Transforming visual data from a camera system or RBG-D camera to 3D skeletons follows the standard approaches in the literature~\cite{XXX,XXX,XXX,XXX}. 


\subsection{Skeleton-Generation Network}
The skeleton generation network takes wireless signals (i.e., horizontal and vertical heatmaps) and generates multi-person 3D skeletons (the yellow box in \autoref{fig:method}). We adopt the top-down detection architecture from \cite{zhao2018rf}. Specifically, the neural network uses spatio-temporal convolutions. Each time, it takes as input a 3-second window of RF signals (90 frames of horizontal and vertical heatmaps). Similar to Faster R-CNN \cite{ren2015faster}, our input first goes through a feature network to extract features from the input RF signals. Since the  convolution operation does not change the spatial distribution of the input, we will obtain two kinds of feature maps, one from the horizontal RF heatmaps and another from vertical RF heatmaps. A region proposal network (RPN) is applied on the horizontal feature maps to obtain several proposals for possible skeleton bounding  boxes. After that, the extracted proposals are fed into a 3D pose estimation subnetwork to extract 3D skeletons from each of them. 

\subsection{Modality-Independent Action Recognition}
After we generate 3D skeletons from raw wireless signals, we can start performing action detection on these skeletons. We first associate the skeletons across time to get multiple skeleton sequences, each from one person. Then we apply our skeleton-based action recognition model to these skeleton sequences.
Our action detection model (the green box in \autoref{fig:method}) has three modules as follows:
1) An attention-based feature learning network, which extracts high-level spatio-temporal features from each skeleton sequence. This module is implemented as a two-stream hierarchical co-occurrence network (HCN) \cite{zhu2016co} that is augmented with spatio-temporal attention.
2) We then pass these features to a multi-proposal module to extract proposals -- i.e., time windows that each corresponds to the beginning and end of an action.  Our multi-proposal module consists of many proposal sub-networks. Each sub-network either takes in features from one person to detect action proposals, or takes in features from two people to detect interaction proposals. (as shown in autoref{fig:method}). 3) Finally, after cropping and resizing the corresponding latent feature using the proposals from our multi-proposal module, we input each cropped action segment into a classification network. The classification network first refines the temporal proposal result by performing a 2-way classification to determine whether this duration contains an action or not. It then predicts the action class of the corresponding action segment.

Nest, we describe the attention module and the multi-proposal module in detail. 


\subsubsection{Spatial-Temporal Attention Module}
Skeletons predicted from wireless signals may not be as accurate as those labeled by humans. Also, different body joints may have different prediction errors. To make our action detection model focus on body joints with higher prediction confidence, we propose a spatial-temporal attention module. Specifically, we define a learnable mask weight $W_m$, and convolve with latent features from spatial path $f_{s}$ and temporal path $f_{t}$ and get the mask to apply on the feature:
$$Mask=Conv(concat(f_{s}, f_{t})).$$ In this way, the mask could learn to provide different weights to different joints to get better action recognition performance. We also add a multi-headed attention module \cite{vaswani2017attention} on the time dimension after the feature extraction to learn the attention on different timestamps.
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{attention}
\caption{\footnotesize{Spatial-temporal attention module to pay different attention on different joints and time segments.}}	\label{fig:rf-heatmaps}
\end{figure}

Our proposed attention module helps the model to learn more representative features, since the learnt mask leverages information provided by both spatial path and temporal path, and the multi-headed attention helps the model to attend more on useful timestamps, while the previous model only have have the two paths interact with each other with late fusion. Our experiments show that the spatial-temporal attention module not only helps increase the action detection accuracy on skeletons predicted from wireless signals, but also helps increase the performance on benchmark visual action recognition datasets. This further shows the proposed attention module helps to combine spatial and temporal representations more effectively, and would lead to better latent representations for the skeleton sequences.

\subsubsection{Multi-Proposal Module} 
Most of previous action recognition datasets have only one action target at a time, regardless of the number of people presented. As a result, previous approaches for skeleton action recognition cannot handle the scenario where multiple people performing different action simultaneously. When there are multiple people in the scene, they typically simply do a max over features extracted from each of them, and forward the resulting combined feature to output one action. Therefore, they can only predict one action label at a time. If one person is sitting while other two people are shaking hands, previous model can not predict both of them.

However, in our dataset, when there are multiple people in the scene, they are free to do any actions or interact with each other at any time. So there are many scenarios where multiple people are doing actions and interacting simultaneously. We tackle this problem with a multi-proposal module. Specifically, denote $N$ to be the number of people appearing at the same time. Instead of performing max-pooling over $N$ features, our multi-proposal module output $N+{n\choose 2}$ proposals from these $N$ features, corresponding to $N$ possible single-person actions and ${n\choose 2}$ possible interactions between each two people. After proposal, we adopt a priority strategy between interact and single person actions. For instance, if there are both predictions for 'pointing to something' (single person) and 'pointing to someone' (interaction) at the same time, our final prediction would be 'pointing to someone'.

Our multi-proposal module enables us to output predicted action for each person at the same time. Also, adding the multi-proposal module will have no harm on previous datasets.

\subsection{Multimodal End-to-end Training}
Since we want to train our model in an end-to-end manner, we can no longer use $\arg\max$ to extract 3D keypoint locations, as in past work on RF-based pose estimation~\cite{zhao2018rf}. Therefore, we use a regressor to perform the function of the $\arg\max$ to extract the exact 3D locations of each keypoint. This makes the whole model differentiable and therefore the action label can also act as a supervision on the skeleton prediction model.

Our end-to-end architecture uses 3D human skeleton as an intermediate representation which makes us able to leverage previous skeleton based action recognition dataset easily. We combine different modalities to train our model in the following manner: For wireless signal datasets, gradients propagate through the whole model, and they are used to tune the parameters of both the skeleton prediction model and the action recognition model; For previous skeleton-based action recognition datasets, the gradients back propagate till the skeleton, and they are used to tune the parameters for the action recognition module. As shown in the experiments section, this multi-modality training significantly increase the data diversity and improves the performance of our model.

==> source/method.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{model}
\end{center}
\caption{Our model architecture. Our model first extract 3D skeleton estimations for each person from raw wireless signal inputs. It then perform action recognition on the extracted skeletons.}\label{fig:method}
\end{figure*}


\section{Methods}

Our model architecture is illustrated in \autoref{fig:method}. It includes two parts: The model first extract 3D skeleton estimations for each person from raw wireless signal inputs. It then use the skeleton to perform action recognition. We now illustrate each part of model in detail.

\subsection{Radio Signal to Skeleton}
We adopt the top-down detection architecture from \cite{zhao2018rf} to generate multi-people's 3D skeleton from RF signals. More specifically, each time we input 3 seconds (90 frames) of RF signals (horizontal and vertical map) into the network. Similar to Faster R-CNN framework \cite{ren2015faster}, our input first go through a feature network to extract features from the input RF signals. Since convolution operation will not change the spatial distribution of the input, we will obtain two kinds of feature maps, one from the horizontal RF heatmaps and another from vertical RF heatmaps. A region proposal network (RPN) is applied on the horizontal feature maps to get several proposals for possible skeleton location. After that, the extracted proposals are fed into a 3D pose estimation subnetwork to extract 3D skeletons from each of them. 

\subsection{Skeleton to Action}
After we generate 3D skeletons from the raw wireless signals, we can start to perform action detection from these skeletons. We first associate the skeletons across time to get multiple skeleton sequences, each from one person. Then we apply our skeleton-based action recognition algorithms on these skeleton sequences. We follow the good practice in \cite{zhu2016co} and adopt their hierarchical co-occurance network to learn high-level latent features to detect actions. Specifically, we leverage the two-stream co-occurance network architecture to extract spatial-temporal features as well as joint co-occurrences. We follow the previous works which extend the Faster R-CNN\cite{girshick2015fast} framework to temporal dimension and adapt it to the task of action detection \cite{zhu2016co}. In the following we will briefly show our action detection model and 
introduce several modules to adapt the model to fit our task of detecting actions from wireless signals. Specifically, after getting high-level features with HCN\cite{zhu2016co}, we connect the feature to a temporal proposal network to extract temporal durations that possibly include an action. After cropping and resizing the corresponding latent feature, we input it into a classification network. The classification network is responsible for two things: First, it will refine the temporal proposal result and do a 2-way classification to determine whether this duration contains an action or not. Second, it will predict the action class of the corresponding temporal duration.

\textbf{Multi-proposal Module} 
Previous approaches for skeleton action recognition cannot handle the scenario where multiple people performing different action simultaneously, since their model can only predict one action label for each duration. If one person is sitting while other other two people are shaking hands, previous model can not predict both actions. We tackle this problem by a multi-proposal module. Specifically, denote $N$ to be the maximum possible number of person appear at the same time. To consider the action for everyone, we first stack all body joints from every person to be the input for our model, for scenario with $<N$ person performing actions, we simply pad zero. After extracting latent features from each one of the skeleton sequences, instead of performing max-pooling over $N$ features, our temporal proposal subnetwork propose $N+C_N^2$, corresponding to $N$ single-person actions and $C_N^2$ possible interactions between different person. After proposal, we adopt a rank pooling strategy between interact and single person actions. For instance, if there are both predictions for 'pointing to something'(single person) and 'pointing to someone'(interaction) at the same time, our final prediction would be 'pointing to someone'.
Our multi-proposal module can be easily adapt to most of the previous action detection frameworks to enable the model to predict multiple actions and interactions at the same time.


\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{attention}
\caption{Spatial-temporal attention module to pay different attention on different joints and time segments. \red{to replace}}	\label{fig:rf-heatmaps}
\end{figure}
\textbf{Spatial-Temporal Attention Module}
Skeletons predicted from wireless signals may not be as accurate as labeled by human. Also, different body joints may have different predict accuracies. To make our action detection model focus more on the body joint with higher prediction confidence, we propose a spatial-temporal attention module(STAM). Specifically, we define a learnable mask weight $W_m$, and convolve with latent features from spatial path $f_{si}$ and temporal path $f_{ti}$ and get the mask to apply on the feature.
$$Mask=Conv(concat(f_{si}, f_{ti}))$$
In this way, the mask could learn to provide different weights to different joints to get better action recognition performance.
In practice, we find the proposed attention module also helps the model to learn more representation features, since the learnt mask leverage information provided by both spatial path and temporal path, while the previous model only have have the two paths interact with each other with late fusion. Therefore, it helps to combine spatial and temporal representations more effectively, and would lead to better latent representations for the skeleton sequences. It could help to classify the actions which can be better disentangled by a mixture of spatial and temporal information, e.g. brushing hair and answering phone.
Our spatial-temporal attention module and also be easily adapted to most of the previous two-stream based neural network architectures for action recognition and other spatial-temporal modeling tasks, and our experiments show that it also helps increase the performance on benchmark action recognition datasets. 


\subsection{Multimodal End-to-end Training}
Our end-to-end architecture has 3D human skeleton as an intermediate representation, which makes us able to leverage previous skeleton based action recognition dataset easily. We train our model with different modalities in the following manner: For wireless signal datasets, gradients propagate through the whole model, and they are used to tune the parameters in both skeleton prediction module and action recognition module; For previous skeleton-based action recognition datasets, the gradients back propagate till the skeleton, and they are used to tune the parameters for the action recognition module. Indeed, datasets for action recognition from other modalities can also be leveraged, as long as we can extract skeletons from the inputs.


==> source/related-1.tex <==
\section{Related Works}
\label{sec:related}

%\subsection{Video -Based Action Recognition}
\noindent {\bf (a)~~Video-Based Activity Recognition: }
Recognizing actions from videos has been a hot topic over the past several years. Early methods use hand-crafted features. For instances, image descriptors like HOG and SIFT have been extended to 3D \cite{chen2009mosift,ng2018actionflownet} to extract temporal clues from videos. Also, descriptors like improved Dense Trajectories (iDT) \cite{wang2013action} are specially designed to track motion information in videos. More recent solutions are based on deep learning, and 
 fall into two main categories. The first category extracts motion and appearance features jointly by leveraging 3D convolution networks \cite{carreira2017quo,qiu2017learning}. Yet, it is computationally expensive to model the video with 3D convolutions. As a result, the second category considers spatial features and temporal features separately by using two-stream neural networks \cite{simonyan2014two, yue2015beyond, wang2016temporal}. Further, it is quite hard to input a whole video in to the model at once; hence, previous methods tried to use a sliding window \cite{xu2017r} to reduce computational overhead.  

%\subsection{Skeleton-Based Action Recognition}
\vskip  0.06in\noindent {\bf (b)~~Skeleton-Based Activity Recognition: }
Recently, skeleton-based action recognition has gained much attention from the research community\cite{fang2017rmpe,cao2018openpose}. Such an approach has multiple advantages. First, skeleton data provide a robust representation for human dynamics against background noises \cite{li2018co}. Second, human skeleton data are more succinct in comparison to RGB videos, which reduces computational overheard and allows for smaller models suitable for mobile platforms \cite{ke2017new}.

Previous methods for action recognition from skeletons can be divided into three categories. Recurrent Neural Networks (RNNs) can model long-term temporal dependencies and therefore have been exploited to process sequences of skeleton data \cite{du2015hierarchical,shahroudy2016ntu,zhu2016co}. However, in recent years, the literature has shifted to Convolutional Neural Networks (CNNs) to learn spatio-temporal features and achieved impressive performance\cite{du2015skeleton,li2018co,ke2017new}. Last, some papers represent human skeletons as graphs and utilize graph neural network (GNN) for action recognition \cite{yan2018spatial, gao2018generalized}. There are also several works combining these strategies for better performance. For example, Si \etal \cite{si2018skeleton} extract spatial-level feature with a Graph Neural Network and leverage LSTM to exploit temporal correlations from the skeleton sequences.

%A limitation of previous skeleton based action recognition is that they con't deal with the scenarios that multiple people doing different actions simultaneously, they can only produce one action label during a certain period of time. Our model tackles this problem by introducing a multi-proposal module. This module would propose multiple temporal windows through time, thus could handle multiple simultaneous actions properly.


%\subsection{Radio-Based Activity Recognition}
\vskip  0.06in\noindent {\bf (c)~~Radio-Based Activity Recognition: }
Research in wireless systems has explored activity recognition using radio signals, particularly for home applications where privacy concerns may preclude the use of cameras ~\cite{wang2014eyes, guo2017novel, pu2013whole, abdelnasser2015wigest}.  This work can be divided into two categories:  The first category is similar to \name\ in that it analyses the radio signals that bounce off people's bodies. They use action labels for supervision, and simple classifiers \cite{wang2014eyes, guo2017novel, pu2013whole, abdelnasser2015wigest}. As a result, current systems can only recognize simple activities such as walking, sitting and running, and the number of different activities is typically limited to less than 10 activities.  The second category relies on a network of sensors. They either use the data collected from multiple sensors across the environment to infer the activities of the subject (e.g., a sensor on the fridge can detect eating) \cite{kasteren2010activity, yang2011activity}, or they track different body parts of a person by attaching radio devices to each of them and recognizing the subject's activities based on the signal from these wearable radios \cite{keally2011pbn}. However, these systems require either significant infrastructure installation or diligent usage of wearable devices, which significantly reduce their utility and robustness.



==> source/related.tex <==
\section{Related Works}
\label{sec:related}

\subsection{Video -Based Action Recognition}
Recognizing actions from videos has been a hot topic over the past several years. Early methods use hand-crafted features to exploit motion features from videos. For instances, image descriptors like HOG and SIFT have been extended to 3D \cite{chen2009mosift,ng2018actionflownet} to extract temporal clues from videos. Also, descriptors like improved Dense Trajectories (iDT) \cite{wang2013action} are specially designed to track the motion information provided with videos.

The success of applying deep learning in image recognition tasks have motivated researchers to apply deep neural networks to the task of video action recognition. Previous works for applying deep learning to action recognition fall into two main categories. The first category extracts motion and appearance features jointly by leveraging 3D convolution networks \cite{carreira2017quo,qiu2017learning}. Yet, it is computationally expensive to model the video with 3D convolution operations. As a result, the second category considers spatial features and temporal features separately by using two-stream neural networks \cite{simonyan2014two, yue2015beyond, wang2016temporal}. However, video data is quite expensive in space. Moreover, most of the previous works on video action recognition include optical-flows as inputs, which takes even more space to store the data. Also, given the size of video data, it is quite hard to input a whole test duration in to the model at one time. Previous methods tried to use a sliding window \cite{xu2017r} to deal with this problem, yet such a design is less accurate and less efficient than inferencing the whole temporal duration at one time.


\subsection{Skeleton-Based Action Recognition}
Recently, skeleton-based action recognition has gained much attention from the research community, as human skeleton extraction performance has been improved significantly by recent approaches \cite{fang2017rmpe,cao2018openpose}. Detecting and recognizing actions from skeletons have many advantages. First, skeleton data provide a robust representation for human dynamics against background noises. It extracts a relatively higher level of motion information for human actions \cite{li2018co}. Second, human skeleton data are much smaller and more succinct comparing to RGB videos. Therefore, it is easier to reduce the model size and to deploy the model on mobile platforms \cite{ke2017new}.

Previous methods for action recognition with skeletons can be divided into three categories. The Recurrent Neural Networks (RNNs) are designed to model long-term temporal dependency problems and therefore are exploited to learn better temporal correlations from sequences of human skeleton data \cite{du2015hierarchical,shahroudy2016ntu,zhu2016co}. However, more and more literature adopted Convolutional Neural Networks (CNNs) to learn skeleton features and achieved impressive performance in recent years \cite{du2015skeleton,li2018co,ke2017new}, as CNN models are equipped with excellent ability to extract spatial-temporal information simultaneously. The third category tries to format the human skeletons as graph-like data and utilize graph neural network to solve this task \cite{yan2018spatial, gao2018generalized}, which is a more natural way to represent skeletons and make more use of the intrinsic human skeleton structure. 

There also have been several works combining these strategies for better performance. Si \etal proposed a spatial reasoning and temporal stack learning approach to combine the power of GCN and RNN \cite{si2018skeleton}. They extracted spatial-level feature with a Graph Neural Network and further leverage LSTM to exploit temporal correlations from the skeleton sequences.

A limitation of previous skeleton based action recognition is that they con't deal with the scenerio that multiple people doing different actions simultaneously, they can only produce one action label during a certain period of time. Our model tackles this problem by introducing a multi-proposal module. This module would propose multiple temporal windows through time, thus could handle multiple simultaneous actions properly.


\subsection{Radio-Based Activity Recognition}
Recent years have witnessed much interest in detecting and recognizing human activities using low-frequency wireless signals. Typically, these signals are with frequency around a few GHz and hence can detect people's activities through walls and occlusions. Such through-wall activity recognition systems can be divided into two categories: device-based systems and device-free systems. 

Device-based systems typically rely on dedicated sensors that are installed in the environment or worn by the tracked subjects. They either use the data collected from sensors across the environment to infer the activities of the subject \cite{kasteren2010activity, yang2011activity}, or track different body parts of a person by attaching radio devices to each of them and recognizing the subject's activities based on the received movements \cite{keally2011pbn}. However, these systems require either significant infrastructure installation or diligent usage of wearable devices, which significantly reduce their utility and robustness.

On the other hand, device-free systems do not require the person to wear sensors on their body or deploy multiple sensors in the environment. They work by analyzing the radio signals reflected off the person's body. However, device-free systems typically have low spatial resolution of the reflected signals, and hence cannot extract enough information for fine-grained activities. As a result, current device-free activity recognition systems can only recognize simple activities such as walking, sitting and running, and the number of different activities is typically limited to less than 10 activities \cite{wang2014eyes, guo2017novel, pu2013whole, abdelnasser2015wigest}.


==> source/rf-1.tex <==
\section{Radio Frequency Signals}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{rf-heatmaps}
\caption{\footnotesize{RF heatmaps and an RGB image recorded at the same time.}}	\label{fig:rf-heatmaps}
\end{figure}

%RF signals share many similarities with visible light, but have lower frequencies. Imaging with RF signals have been used for many decades in the radar industry. Further airport scanners image the human body with radio signals to detect metallic objects. But RF signals also differ from visible light in important ways. They traverse opaque objects, such as wall and most occlusions, which make them complementary to cameras. 

We use a type of radio commonly used in past work on RF-based action recognition~\cite{zhao2018rf,soli, https://ieeexplore.ieee.org/abstract/document/8300506, http://discovery.ucl.ac.uk/1535165/7/Chetty_1018808.pdf, https://ieeexplore.ieee.org/document/7540121, Aryokee}.  The radio generates a waveform called FMCW and operates between 5.4 and 7.2 GHz. The device has two arrays of antennas organized vertically and horizontally. By measuring the signal reflections at the two arrays, the device can create a two-dimensional heatmap, one from the horizontal array and one from the vertical array. As shown in \autoref{fig:rf-heatmaps}, the horizontal heatmap is a projection of the  radio signal on a plane parallel to the ground, whereas the vertical heatmap is a projection of the signal on a plane perpendicular to the ground (red refers to large values while blue refers to small values). %Note that since RF signals are complex numbers, each pixel in this map has a real and imaginary components. 
Intuitively, higher values correspond to higher strength of signal reflections from a location.
The radio works at a frame rate of 30 FPS, i.e., it generates 30 pairs of heatmaps per second. 

As shown in \autoref{fig:rf-heatmaps}, RF signals have very different properties than visual data, which makes RF-based action recognition a difficult problem. Here we list some of those properties that are challenging for RF-based action recognition.
\begin{Itemize}
	\item First, RF signals in the frequencies that traverse walls have much lower spatial resolution than visual data. For our system, the depth resolution is about 10 cm, and the angle resolution is about 10 degrees. This low resolution makes it hard to distinguish similar activities such as hand waving versus brushing hair.
	\item Second, the human body is specular in the frequency range that traverse walls \cite{beckmann1987scattering}. RF specularity is a physical phenomenon that occurs when the wavelength is larger than the roughness of the surface. In this case, the object acts like a reflector - i.e., a mirror - as opposed to a scatterer. The wavelength of our radio is about 5cm and hence humans act as reflectors. Depending on the orientation of the surface of each limb, the signal may be reflected towards our sensor or away from it. Limbs that reflect the signal away from the radio become invisible for the device. Even if the signals are reflected back to the radio, limbs with a small surface (e.g., hands) reflect less signal and hence are harder to track. 
	\item Third, RF signals will attenuate when they traverse walls or occlusions. Although RF signals at low frequency band can go through walls, the attenuation will be significantly larger than through air. As a result, the RF signals reflected from human body can be more vague when the person is behind a wall, and hence the accuracy of detecting an action decreases in the presence of walls and occlusions. 
\end{Itemize}



==> source/rf.tex <==
\section{Radio Frequency Signals}

\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{rf-heatmaps}
\caption{RF heatmaps and an RGB image recorded at the same time. \red{to replace}}	\label{fig:rf-heatmaps}
\end{figure}

In this section, we briefly introduce the radio frequency signals we use for our through-wall action recognition task. Our device uses RF signals with frequency band sweeping from 5.4 to 7.2 GHz, close to the bands of WiFi networks. The transmission power is less than one millie Watt. Similar with many radar systems, our device senses the world by transmitting a low power RF signal and receiving its reflections. To separate RF reflections from different directions and depth, we use common techniques: FMCW (Frequency Modulated Continuous Wave) and antenna arrays \cite{adib2015capturing}. FMCW separates RF reflections based on the distance of the reflecting object, whereas antenna arrays separate reflections based on their spatial direction. 

In this paper, we introduce a radio similar to \cite{zhao2018rf}, which generates an FMCW signal and has two antenna arrays: vertical and horizontal. Thus, our input data takes the form of two-dimensional heatmaps, one from the horizontal array and one from the vertical array. As shown in \autoref{fig:rf-heatmaps}, the horizontal heatmap is a projection of the signal reflections on a plane parallel to the ground, whereas the vertical heatmap is a projection of the reflected signals on a plane perpendicular to the ground (red refers to large values while blue refers to small values). Note that since RF signals are complex numbers, each pixel in this map has a real and imaginary components. Our radio works in a frame rate of 30 FPS, which means that it generates 30 pairs of heatmaps per second. 


As shown in \autoref{fig:rf-heatmaps}, RF signals have very different properties than visual data, which makes RF-based action recognition a long-lasting open-problem in RF community. Here we list some of those properties that are challenging for RF-based action recognition.
\begin{itemize}
	\item First, RF signals in the frequencies that traverse walls have much lower spatial resolution than visual data. For our system, the depth resolution from FMCW is about 10 cm, and the angle resolution from antenna array is about 10 degrees. This low resolution makes it hard to distinguish similar activities such as hand waving versus brushing hair.
	\item Second, the human body is specular in the frequency range that traverse walls \cite{beckmann1987scattering}. RF specularity is a physical phenomenon that occurs when the wavelength is larger than the roughness of the surface. In this case, the object acts like a reflector - i.e., a mirror - as opposed to a scatterer. The wavelength of our radio is about 5cm and hence humans act as reflectors. Depending on the orientation of the surface of each limb, the signal may be reflected towards our sensor or away from it. Even if the signals are reflected back, the limbs with small sizes (e.g., hand and arm) which is necessary for action recognition will reflect much less signals than the torso, making it much harder to localize them.
	\item Third, RF signals will attenuate when it traverse through walls or occlusions. Although RF signals at low frequency band can go through wall, the attenuation will be much larger than what it faced with when travels through air. As a result, the RF signals reflected from human body can be more vague when the person is behind a wall, and hence much harder for through-wall action recognition.
\end{itemize}


